A Model Counter's Guide to Probabilistic Systems

In this paper, we systematize the modeling of probabilistic systems for the purpose of analyzing them with model counting techniques. Starting from unbiased coin flips, we show how to model biased coins, correlated coins, and distributions over finite sets. From there, we continue with modeling sequential systems, such as Markov chains, and revisit the relationship between weighted and unweighted model counting. Thereby, this work provides a conceptual framework for deriving #SAT encodings for probabilistic inference.

==> sections/case_studies.tex <==
\section{Case Study: Learning from Demonstrations}
We conclude with a small example, motivated by the problem of learning
bounded trace properties from unlabeled demonstrations.  For a
detailed explanation of the technique, we refer the readers
to~\cite{vc}.  For our purposes it suffices to know that the maximum
entropy likelihood assigned to a property, $\f$, over an episode of
length $\tau$, is the information gain (KL divergence) of the biased
coin induced by composing agents policy, the dynamics, and the monitor
for $\f$, over the biased coin induced by using a (uniformly) random
action policy. As this example, is meant to be illustrative, we shall
focus on computing the random satisfaction probability.
\begin{wrapfigure}{r}{0.25\textwidth}
   \begin{center}
     \includegraphics[width=\linewidth]{imgs/gridworld.png}
      \caption{\label{fig:gridworld}}
  \end{center}
\end{wrapfigure}
~~~~~~For concreteness, consider an robot operating in the 2d gridworld
illustrated in Fig~\ref{fig:gridworld} for $10$ time steps. The robot
can apply actions for moving in the four cardinal directions (north,
south, east, west); however, with some probability the agent will slip
and move in a random direction. Further, if the agent enters a lava
(red) tile, there is some probability that the agent will transition
into a fail (sink) state. The task specification is to reach any
of the yellow (recharge) tiles without touching a red tile (lava).
Additionally, if a blue tile (water) is stepped on, the agent must
step on a brown tile (drying tile) before going to a yellow tile. Next,
we shall sketch how to encode the task into a model counting query.

To begin, observe that our 2d gridworld can be viewed as two 1d
gridworlds (recall Fig.~\ref{fig:chain} from Ex~\ref{ex:sailor}) whose
actions are correlated, e.g., exactly one of the 1d gridworlds moves
per time step. Further, as there are only $4$ actions, the random
action policy corresponds to the identity map, $\text{id} : \Bool^2
\to \Bool^2$. Finally, observe that the property can be expressed as a
short past tense temporal logic property, and can thus be encoded as a
simple sequential circuit~\cite{ltl2circ}. Denoting by $C$ the circuit that
results from composing the policy, dynamics, and monitor, the random
satisfaction probability is given by:


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../root"
%%% End:  
